Conflict-Based Search for Explainable Multi-Agent Path Finding

In the Multi-Agent Path Finding (MAPF) problem, the goal is to find non-colliding paths for agents in an environment, such that each agent reaches its goal from its initial location. In safety-critical applications, a human supervisor may want to verify that the plan is indeed collision-free. To this end, a recent work introduces a notion of explainability for MAPF based on a visualization of the plan as a short sequence of images representing time segments, where in each time segment the trajectories of the agents are disjoint. Then, the explainable MAPF problem asks for a set of non-colliding paths that admits a short-enough explanation. Explainable MAPF adds a new difficulty to MAPF, in that it is NP-hard with respect to the size of the environment, and not just the number of agents. Thus, traditional MAPF algorithms are not equipped to directly handle explainable-MAPF. In this work, we adapt Conflict Based Search (CBS), a well-studied algorithm for MAPF, to handle explainable MAPF. We show how to add explainability constraints on top of the standard CBS tree and its underlying A* search. We examine the usefulness of this approach and, in particular, the tradeoff between planning time and explainability.

==> Sections/Table.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{|C|CC|CCC|CCCC|CCCC|} % putting table in math mode so we do not need $$ everywhere. Putting headers in \text format
\hline
 & & & \multicolumn{3}{c}{\shortstack{\\CBS}} & \multicolumn{4}{|c|}{XG-CBS w/ $A^*$} & \multicolumn{4}{c|}{XG-CBS w/ XG-$A^*$}\\
\hline
 & \text{\shortstack{\\ \#\\ Agents}} & \text{\shortstack{Grid\\ Size}} & \text{\shortstack{Runtime \\ (s)}}   & \text{\shortstack{Tree\\ Size}} & \text{Index} & r      & \text{\shortstack{Runtime \\ (s)}}  & \text{\shortstack{Tree\\ Size}} & \text{Index} & r                          & \text{\shortstack{Runtime \\ (s)}}  & \text{\shortstack{Tree\\ Size}} & \text{Index} \\
 \hline
1   & 4     & 9\times9    & 0.002     & 3     & 5     & 4     & 0.005     & 5     & 3     & 4     & 0.003     & 3    & \mathbf{2}      \\
2   & 4     & 9\times9    & 0.002     & 3     & 4     & 3     & 0.003     & 1     & 3     & 2     & 0.014     & 2    & \mathbf{2}      \\
3   & 4     & 9\times9    & 0.001     & 1     & 3     & 2     & 0.003     & 1     & 2     & 1     & 0.039     & 15   & \mathbf{1}      \\
4   & 4     & 9\times9    & 0.01      & 21    & 7     & 5     & 0.029     & 40    & 5     & 2     & 0.86      & 24   & \mathbf{2}      \\
\hline
5   & 8     & 9\times9    & 0.013     & 11    & 5     & 4     & -         &  -    & -     & 4     & 0.495    & 5     & \mathbf{4}     \\
6   & 8     & 9\times9    & 0.006     & 7     & 6     & 4     & 0.033     & 54    & \mathbf{4}     & 4     & 1.3       & 10    & 4     \\
7   & 8     & 9\times9    & 0.005     & 5     & 6     & 5     & 0.015     & 12    & 4     & 2     & 128.1     & 105   & \mathbf{2}     \\
\hline
8   & 8     & 16\times16   & 0.119     & 3     & 6     & 4     & 1.9       & 121   & \mathbf{4}     & 5     & 0.3       & 3     & 5     \\
9   & 8     & 16\times16   & 0.0483    & 7     & 6     & 4     & 0.548     & 94    & \mathbf{4}     & 5     & 2         & 3     & 5     \\
10  & 8     & 16\times16   & 0.111     & 3     & 6     & 2     & 0.44      & 69    & \mathbf{2}     & 5     & -         & -     & -     \\
\hline
11  & 8     & 21\times21   & 0.109     & 1     & 5     & 4     & 0.195     & 9     & 3     & 4     & 113.9     & 1     & \mathbf{2}     \\
12  & 8     & 21\times21   & 0.636     & 13    & 7     & 4     & 2.8       & 59    & \mathbf{4}     & 6     &  -        & -    & -      \\
\hline
13  & 9     & 26\times26   & 0.383     & 7     & 6     & 3     & 0.815     & 17    & \mathbf{3}     & 5     & 265.9     & 8     & 4     \\
14  & 9     & 26\times26   & 0.748     & 9     & 9     & 5     & 22.2      & 319   & \mathbf{5}     & 8     & 432.7     & 5     & 5     \\
15  & 9     & 26\times26   & 0.409     & 3     & 8     & 5     & 3.5       & 51    & 5     & 2     & 561.1     & 210   & \mathbf{2}     \\
\hline
16  & 10    & 33\times33  & 0.72      & 3     & 6     & 5     & 1.6       & 15    & \mathbf{3}     & 5     & 38.5      & 1     & 4     \\
17  & 10    & 33\times33  & 0.522     & 1     & 5     & 3     & 3.2       & 26    & \mathbf{3}     & 3     & 341.8     & 18    & 3     \\
18  & 10    & 33\times33  & 1.2       & 1     & 17    & 8     & 14        & 89    & \mathbf{8}     & 16    & 743.7     & 1     & 13    \\ 
19  & 10    & 33\times33  & 0.522     & 1     & 6     & 4     & 5.9       & 89    & \mathbf{4}     & 5     & -         & -     & -     \\
20  & 10    & 33\times33  & 0.721     & 1     & 8     & 5     & 42.1    & 446   & \mathbf{5}     & 7     & -         & -     & -     \\
21  & 10    & 33\times33  & 0.82      & 7     & 7     & 4     & 162.1     & 2421  & \mathbf{4}     & 6     & -         & -     & -     \\
\hline
22  & 12    & 33\times33  & 0.455     & 3     & 6     & 3     & 2.4       & 48    & \mathbf{3}     & 5     & -         & -     & -     \\
23  & 12    & 33\times33  & 5.2       & 35    & 13    & 5     & 126.1     & 1068  & \mathbf{5}     & 12    & -         & -     & -     \\
24  & 12    & 33\times33  & 7.3       & 129   & 22    & 10    & 357.6     & 3966  & \mathbf{10}    & 21    & -         & -     & -     \\
\hline
\end{tabular}
  \captionof{table}{Benchmark results for $24$ MAPF instances, grouped into $7$ categories based on the number of agents and grid size. The minimal-index plan found for each planner is shown (the lowest index is in bold).}
  \label{tab:table_benchmark}
\end{table*}
